Finding Needles in Emb(a)dding Haystacks: Legal Document Retrieval via Bagging and SVR Ensembles

We introduce a retrieval approach leveraging Support Vector Regression (SVR) ensembles, bootstrap aggregation (bagging), and embedding spaces on the German Dataset for Legal Information Retrieval (GerDaLIR). By conceptualizing the retrieval task in terms of multiple binary needle-in-a-haystack subtasks, we show improved recall over the baselines (0.849 > 0.803 | 0.829) using our voting ensemble, suggesting promising initial results, without training or fine-tuning any deep learning models. Our approach holds potential for further enhancement, particularly through refining the encoding models and optimizing hyperparameters.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> citation.tex <==
@inproceedings{Boenisch:et:al:2024,
	title        = {Finding Needles in Emb(a)dding Haystacks: Legal Document Retrieval via Bagging and SVR Ensembles},
	author       = {B\"{o}nisch, Kevin and Mehler, Alexander},
	year         = 2024,
	booktitle    = {Proceedings of the 2nd Legal Information Retrieval meets Artificial Intelligence Workshop LIRAI 2024},
	location     = {Poznan, Poland},
	publisher    = {CEUR-WS.org},
	address      = {Aachen, Germany},
	series       = {CEUR Workshop Proceedings},
	note         = {accepted},
	abstract     = {We introduce a retrieval approach leveraging Support Vector Regression (SVR) ensembles, bootstrap aggregation (bagging), and embedding spaces on the German Dataset for Legal Information Retrieval (GerDaLIR). By conceptualizing the retrieval task in terms of multiple binary needle-in-a-haystack subtasks, we show improved recall over the baselines (0.849 > 0.803 | 0.829) using our voting ensemble, suggesting promising initial results, without training or fine-tuning any deep learning models. Our approach holds potential for further enhancement, particularly through refining the encoding models and optimizing hyperparameters.},
	keywords     = {legal information retrieval, support vector regression, word embeddings, bagging ensemble}
}


==> tex/eda-fig-2.tex <==

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.496\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/sentences/deBERTa_base_10k_sentences.png}
        \caption*{\footnotesize a) deBERTa\_base chunked}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.496\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/sentences/deBERTA_base_longformer_10k_sentences.png}
        \caption*{b) Longformer\_base chunked}
    \end{subfigure}
    \caption{Exemplary TSNE plots of the same embedding spaces shown in \Autoref{fig:eda-2}, with the addition of chunking the passages into segments of similar lengths matching their overall average length, demonstrate that the average distance to the most relevant passage of each query is smaller compared to the spaces without chunking.}
    \label{fig:eda-2}
\end{figure}
